A Generic On-Board AI Processing Chain for Earth Observation: From Application Development to Embedded Deployment and Mission-Level Orchestration

Earth observation satellites acquire more data than they can downlink. Extracting information on board with artificial intelligence (AI) turns the satellite into a data-reduction stage that downlinks compact products, such as masks or detections, instead of full scenes; deploying it in a mission, however, involves the whole processing chain and not only the neural network. We present a generic on-board AI processing chain along three axes, with wildfire segmentation as the worked example among ship detection and cloud segmentation. (i) The AI model is tuned (spectral-band selection, input normalization), quantized to 8-bit integers (int8) and ported to an AMD Versal VCK190, with its excellent segmentation performance preserved on the board. (ii) A modular tiler-inference-mosaicer workflow, reused unchanged across applications, brings the tile-level model to scene level, turning a full acquisition into a scene-level mask or detection list. (iii) Each step is packaged as a unikernel and orchestrated on board by ORCHIDE, a cloud-native orchestrator. The chain is characterized end to end, from the standalone execution on the target to its execution under orchestration with parallel workflows on a representative test bench. Beyond AI inference on individual tiles, this approach aims at increasing the maturity of on-board AI deployment by addressing a complete processing chain, from the acquired scene to the mission-level execution.

==> Makefile <==
# ============================================================
#  OBPDC 2026 paper -- arXiv branch (ceos_arxiv)
#
#  main.tex is self-contained (sections, TikZ figure and
#  bibliography inlined): no \input, no BibTeX.
#  make        -> main.pdf
#  make clean  -> remove build artifacts
# ============================================================

MAIN  = main
LATEX = pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all pdf clean

all: pdf

pdf: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(wildcard figures/*)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)

clean:
	rm -f $(MAIN).aux $(MAIN).log $(MAIN).out $(MAIN).toc

